A Contrario multi-scale anomaly detection method for industrial quality inspection

Anomalies can be defined as any non-random structure which deviates from normality. Anomaly detection methods reported in the literature are numerous and diverse, as what is considered anomalous usually varies depending on particular scenarios and applications. In this work we propose an a contrario framework to detect anomalies in images applying statistical analysis to feature maps obtained via convolutions. We evaluate filters learned from the image under analysis via patch PCA, Gabor filters and the feature maps obtained from a pre-trained deep neural network (Resnet). The proposed method is multi-scale and fully unsupervised and is able to detect anomalies in a wide variety of scenarios. While the end goal of this work is the detection of subtle defects in leather samples for the automotive industry, we show that the same algorithm achieves state-of-the-art results in public anomalies datasets.

==> plot_cracks.tex <==
% \vspace{-10pt}
\captionsetup{position=top}
\begin{figure}[tb]

\subfloat[]{\includegraphics[width=0.138\linewidth]{pics/cracks/images/001_0000.jpg}} \hfill
\subfloat[]{\includegraphics[width=0.138\linewidth]{pics/cracks/labels/001_0000.jpg}} \hfill
\subfloat[]{\includegraphics[width=0.138\linewidth]{pics/cracks/ours_blob_gabor/001_0000.jpg}} \hfill
\subfloat[]{\includegraphics[width=0.138\linewidth]{pics/cracks/drfi/001_0000.jpg}} \hfill
\subfloat[]{\includegraphics[width=0.138\linewidth]{pics/cracks/gbvs/001_0000.jpg}} \hfill
\subfloat[]{\includegraphics[width=0.138\linewidth]{pics/cracks/salicon/001_0000.jpg}} \hfill
\subfloat[]{\includegraphics[width=0.138\linewidth]{pics/cracks/allterrain_augmented/001_0000.jpg}} \hfill \\[-20px]

\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/images/001_0003.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/labels/001_0003.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/ours_blob_gabor/001_0003.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/drfi/001_0003.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/gbvs/001_0003.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/salicon/001_0003.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/allterrain_augmented/001_0003.jpg}} \hfill \\[-20px]

\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/images/001_0007.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/labels/001_0007.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/ours_blob_gabor/001_0007.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/drfi/001_0007.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/gbvs/001_0007.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/salicon/001_0007.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/allterrain_augmented/001_0007.jpg}} \hfill \\[-20px]

\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/images/024_0008.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/labels/024_0008.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/ours_blob_gabor/024_0008.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/drfi/024_0008.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/gbvs/024_0008.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/salicon/024_0008.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/allterrain_augmented/024_0008.jpg}} \hfill \\[-20px]

\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/images/030_0002.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/labels/030_0002.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/ours_blob_gabor/030_0002.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/drfi/030_0002.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/gbvs/030_0002.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/salicon/030_0002.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/allterrain_augmented/030_0002.jpg}} \hfill \\[-20px]

\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/images/054_0003.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/labels/054_0003.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/ours_blob_gabor/054_0003.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/drfi/054_0003.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/gbvs/054_0003.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/salicon/054_0003.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/allterrain_augmented/054_0003.jpg}} \hfill \\[-20px]

    \caption{Comparison of different method over the Cracks Dataset. (a) image, (b) label, (c) ours, (d) DRFI, (e) GBVS, (f) SALICON, (g) All Terrain}
    \vspace{-10pt}
    \label{fig:results-cracks}
\end{figure}
\captionsetup{position=bottom}

==> plot_ipol.tex <==
\vspace{-10pt}
\captionsetup{position=top}
\begin{figure}[tb]

\subfloat[]{\includegraphics[width=0.162\linewidth]{pics/ipol/images/55fff9bfc4007c65aaff1b2cad9237a411e703bd.jpg}} \hfill
\subfloat[]{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_nfa/55fff9bfc4007c65aaff1b2cad9237a411e703bd.jpg}} \hfill
\subfloat[]{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_det/55fff9bfc4007c65aaff1b2cad9237a411e703bd.jpg}} \hfill
\subfloat[]{\includegraphics[width=0.162\linewidth]{pics/ipol/drfi/55fff9bfc4007c65aaff1b2cad9237a411e703bd.jpg}} \hfill
\subfloat[]{\includegraphics[width=0.162\linewidth]{pics/ipol/gbvs/55fff9bfc4007c65aaff1b2cad9237a411e703bd.jpg}} \hfill
\subfloat[]{\includegraphics[width=0.162\linewidth]{pics/ipol/salicon/55fff9bfc4007c65aaff1b2cad9237a411e703bd.jpg}} \hfill \\[-20px]

\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/images/693ca1ea0ca72e9d2c81e3ae5909314ca00cb0b7.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_nfa/693ca1ea0ca72e9d2c81e3ae5909314ca00cb0b7.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_det/693ca1ea0ca72e9d2c81e3ae5909314ca00cb0b7.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/drfi/693ca1ea0ca72e9d2c81e3ae5909314ca00cb0b7.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/gbvs/693ca1ea0ca72e9d2c81e3ae5909314ca00cb0b7.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/salicon/693ca1ea0ca72e9d2c81e3ae5909314ca00cb0b7.jpg}} \hfill \\[-20px]

\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/images/785e7cf1731258e05e4cf843bea1ffcd3ddc52a7.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_nfa/785e7cf1731258e05e4cf843bea1ffcd3ddc52a7.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_det/785e7cf1731258e05e4cf843bea1ffcd3ddc52a7.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/drfi/785e7cf1731258e05e4cf843bea1ffcd3ddc52a7.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/gbvs/785e7cf1731258e05e4cf843bea1ffcd3ddc52a7.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/salicon/785e7cf1731258e05e4cf843bea1ffcd3ddc52a7.jpg}} \hfill \\[-20px]

\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/images/9c577c528e24499626b18e60584bdb00a776827e.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_nfa/9c577c528e24499626b18e60584bdb00a776827e.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_det/9c577c528e24499626b18e60584bdb00a776827e.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/drfi/9c577c528e24499626b18e60584bdb00a776827e.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/gbvs/9c577c528e24499626b18e60584bdb00a776827e.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/salicon/9c577c528e24499626b18e60584bdb00a776827e.jpg}} \hfill \\[-20px]

\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/images/bird.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_nfa/bird.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_det/bird.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/drfi/bird.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/gbvs/bird.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/salicon/bird.jpg}} \hfill \\[-20px]

\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/images/d779a25c72c3f3318d1402af822068ceb7a5c5ae.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_nfa/d779a25c72c3f3318d1402af822068ceb7a5c5ae.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_det/d779a25c72c3f3318d1402af822068ceb7a5c5ae.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/drfi/d779a25c72c3f3318d1402af822068ceb7a5c5ae.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/gbvs/d779a25c72c3f3318d1402af822068ceb7a5c5ae.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/salicon/d779a25c72c3f3318d1402af822068ceb7a5c5ae.jpg}} \hfill \\[-20px]

\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/images/e634e2f23efae2af8447a5a29ef1a979f8a317fe.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_nfa/e634e2f23efae2af8447a5a29ef1a979f8a317fe.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_det/e634e2f23efae2af8447a5a29ef1a979f8a317fe.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/drfi/e634e2f23efae2af8447a5a29ef1a979f8a317fe.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/gbvs/e634e2f23efae2af8447a5a29ef1a979f8a317fe.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/salicon/e634e2f23efae2af8447a5a29ef1a979f8a317fe.jpg}} \hfill \\[-20px]

\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/images/f4252df6758563293bdbc6a7db346bbb922778cf.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_nfa/f4252df6758563293bdbc6a7db346bbb922778cf.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_det/f4252df6758563293bdbc6a7db346bbb922778cf.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/drfi/f4252df6758563293bdbc6a7db346bbb922778cf.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/gbvs/f4252df6758563293bdbc6a7db346bbb922778cf.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/salicon/f4252df6758563293bdbc6a7db346bbb922778cf.jpg}} \hfill \\[-20px]

\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/images/field3_bw.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_nfa/field3_bw.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_det/field3_bw.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/drfi/field3_bw.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/gbvs/field3_bw.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/salicon/field3_bw.jpg}} \hfill \\[-20px]
    
    \caption{Comparison of the same methods mentioned over sample interesting images (excluding All Terrain algorithm, which was specific for cracks). (a) image, (b) Our NFA map, (c) Our segmentation using NFA=0 as threshold, (d) DRFI, (e) GBVS, (f) SALICON}
    \vspace{-10pt}
    \label{fig:results-ipol}
\end{figure}
\captionsetup{position=bottom}
